Limiting distributions of conjugate algebraic integers

Let $\Sigma \subset \mathbb{C}$ be a compact subset of the complex plane, and $\mu$ be a probability distribution on $\Sigma$. We give necessary and sufficient conditions for $\mu$ to be the weak* limit of a sequence of uniform probability measures on a complete set of conjugate algebraic integers lying eventually in any open set containing $\Sigma$. Given $n\geq 0$, any probability measure $\mu$ satisfying our necessary conditions, and any open set $D$ containing $\Sigma$, we develop and implement a polynomial time algorithm in $n$ that returns an integral monic irreducible polynomial of degree $n$ such that all of its roots are inside $D$ and their root distributions converge weakly to $\mu$ as $n\to \infty$. We also prove our theorem for $\Sigma\subset \mathbb{R}$ and open sets inside $\mathbb{R}$ that recovers Smith's main theorem \cite{Smith} as special case. Given any finite field $\mathbb{F}_q$ and any integer $n$, our algorithm returns infinitely many abelian varieties over $\mathbb{F}_q$ which are not isogenous to the Jacobian of any curve over $\mathbb{F}_{q^n}$.

==> real.tex <==
\subsection{Finding Square-free Polynomials}\label{square_free}
We see in section \ref{int_poly} that Theorem \ref{smith_3_2} requires a square-free polynomial $P$ to get the basis $\mathcal O$. To do this, we need to find monic, square-free integer polynomials of a given degree. Furthermore, we want this polynomial to have a small $n$-norm. The reason for this is that applying Theorem \ref{smith_3_2} gives a polynomial close to the original polynomial in the $n$-norm metric. This is justified in Corollary 3.3 in Smith. Since we know that the basis we created in Section \ref{lattice_bases} is short and has small $n$-norm, we can take a small linear-combination of these basis vectors to get a square-free polynomial of small norm. In practice, we can simply take a degree $n$-polynomial from this basis since it will usually be square-free.
\newline

\subsection{Chebyshev Polynomials}\label{cheb}
Here we discuss the implementation of Proposition 4.1 in Smith. The idea of this proposition is to construct an oscillatory monic polynomial $Q$ given another real monic polynomial $P$ such that $PQ$ has $\deg(Q)$ of the highest degree coefficients being even (after the highest order term). \textcolor{red}{Explain why the oscillation is important. The oscillation forces $Q$ to have all of its roots in our interval $I$ and also that when we approximate with Theorem \ref{smith_3_2}, the number of roots in $I$ does not change}.
\newline

The way we achieve this is with Chebyshev polynomials. Given an interval $I$ with capacity $\kappa$, there is a unique polynomial $f$ of degree $n$ which achieves $\max |f(x)|=2\kappa^r$ precisely $n+1$ times where $\kappa$ is the capacity of $I$. We will call this the Chebyshev polynomial on interval $I$. \textcolor{red}{A proof for this can be seen in Lemma 4.3 of Smith}. We algorithmically compute $Q$ as described above in the manner suggested in Smith's proof of Proposition 4.1 in Smith.

\subsection{Main Algorithm}
First, we find the short square-free, integer polynomial as described in section \ref{square_free}. We then find polynomial $Q$ of degree $m$ (\textcolor{red}{explain where $m$ comes from}) as described in section \ref{cheb} using $P=\tilde{P}_{\mu,n+2}$. Suppose
$$PQ=x^{n+m}+a_{n+m-1}x^{n+m-1}+\dots+a_nx^n+b_{n-1}x^{n-1}+\dots+b_0$$
where all of the $a_i$'s are even integers. Then apply the algorithm discussed in section \ref{int_poly} to $\frac{1}{4}\left(\sum_{i=0}^nb_ix^i\right)+\frac{1}{2}$ get an integer polynomial $H$ close to the original. Finally,
$$x^{n+m}+a_{n+m-1}x^{n+m-1}+\dots+a_nx^n+4H-2$$
is an Eisenstein polynomial at $2$ close in $(n+m)$-norm to $PQ$. If the norm between $PQ$ and the Eisenstein polynomial is small enough, the roots are forced to remain inside $I$.
